PatchRefiner: Leveraging Synthetic Data for Real-Domain High-Resolution Monocular Metric Depth Estimation

This paper introduces PatchRefiner, an advanced framework for metric single image depth estimation aimed at high-resolution real-domain inputs. While depth estimation is crucial for applications such as autonomous driving, 3D generative modeling, and 3D reconstruction, achieving accurate high-resolution depth in real-world scenarios is challenging due to the constraints of existing architectures and the scarcity of detailed real-world depth data. PatchRefiner adopts a tile-based methodology, reconceptualizing high-resolution depth estimation as a refinement process, which results in notable performance enhancements. Utilizing a pseudo-labeling strategy that leverages synthetic data, PatchRefiner incorporates a Detail and Scale Disentangling (DSD) loss to enhance detail capture while maintaining scale accuracy, thus facilitating the effective transfer of knowledge from synthetic to real-world data. Our extensive evaluations demonstrate PatchRefiner's superior performance, significantly outperforming existing benchmarks on the Unreal4KStereo dataset by 18.1% in terms of the root mean squared error (RMSE) and showing marked improvements in detail accuracy and consistent scale estimation on diverse real-world datasets like CityScape, ScanNet++, and ETH3D.

==> tables/abl_weight.tex <==





\begin{table*}[t!]
    \centering
    \caption{\textbf{Impact of Varying DSD Loss Weights.} Increasing the weight slightly reduces scale accuracy while markedly enhancing detail resolution, demonstrating the efficacy of our DSD loss in balancing detail enhancement and scale accuracy.}
    \label{tab:abl-weight}
    % \small
    \scalebox{0.82}{
    \begin{tabular}{cc|*{3}{C{1.8cm}}|*{3}{C{1.8cm}}}
        \toprule
        \multicolumn{2}{c|}{Weight} & \multicolumn{3}{c|}{Scale} & \multicolumn{3}{c}{Boundary} \\
        \cmidrule{1-8}
        
        $\mathcal{L}_{rank}$ & $\mathcal{L}_{ssi}$ & \boldsymbol{$\delta_1 (\%)$}$\uparrow$ &  \textbf{REL}$\downarrow$ & \textbf{RMS}$\downarrow$  & \textbf{Precision}$\uparrow$ & \textbf{Recall}$\uparrow$ & \textbf{F1}$\uparrow$  \\
        \midrule
        
        
        
        \midrule
        
        % 3e$^{-1}$ & 1e$^{-1}$ & 95.329 & 0.067 & 4.044 & 19.02 & 52.83 & 27.57\\ 
        % 1e$^{-1}$ & 3e$^{-1}$ & 95.371 & 0.067 & 4.033 & 20.17 & 50.51 & 28.43 \\ 
        % 3e$^{-2}$ & 1e$^{-1}$ & 95.452 & 0.066 & 3.963 & 18.59 & 44.64 & 25.83 \\ 
        % 1e$^{-1}$ & 3e$^{-2}$ & 95.411 & 0.066 & 3.976 & 18.47 & 48.07 & 26.26 \\ 
        % \midrule
        
        \multicolumn{2}{c|}{PR. $\mathcal{S}$} & 5.705 & 0.399 & 12.20 & 28.68 & 51.28 & 36.34 \\ 
        \multicolumn{2}{c|}{PR. $\mathcal{R}$} & 95.418 & 0.065 & 3.992 & 17.09 & 40.92 & 23.68 \\ 
        
        \bottomrule
    \end{tabular}
    }
\end{table*}


